Automated Code Editing with Search-Generate-Modify

Code editing is essential in evolving software development. Many automated code editing tools have been proposed that leverage both Information Retrieval-based techniques and Machine Learning-based code generation and code editing models. Each technique comes with its own promises and perils, and they are often used together to complement their strengths and compensate for their weaknesses. This paper proposes a hybrid approach to better synthesize code edits by leveraging the power of code search, generation, and modification. Our key observation is that a patch obtained by search and retrieval, even if imperfect, can provide helpful guidance to a code generation model. However, a retrieval-guided patch produced by a code generation model can still be a few tokens off from the intended patch. Such generated patches can be slightly modified to create the intended patches. SARGAM is a novel tool designed to mimic a real developer's code editing behavior. Given an original code version, the developer may search for related patches, generate or write the code, and then modify the generated code to adapt it to the right context. Our evaluation of SARGAM on edit generation shows superior performance with respect to current state-of-the-art techniques. SARGAM also shows great effectiveness on automated program repair tasks.

==> body/1.introduction.back.tex <==
\section{Introduction}

Software developers frequently work on source code in stages, making little modifications throughout the coding process for a variety of reasons, including adding new functionality, resolving bugs, and refactoring. Many of these code patches follow predictable edit patterns, prompting a surge in research into automated code generation based on previous patches. In the past several years, approaches to effectively fix and maintain software have been thoroughly researched in order to decrease developer workload.

Automated Program Repair (APR) methods, which are designed to reduce the manual labor required to address software bugs, have become a hot research topic in the software engineering community in the past decade \cite{monperrusaprbib}. Recent techniques in the literature have shown great potential to automatically correct an increasing number of benchmark bugs. These innovations promise a great deal to the software engineering industry, mainly a significant reduction in downtime, time-to-fix delays, and decreased debugging time with the suggestion of possible fixes.

The current literature mainly centers around code generation and editing, but not patch retrieval. This is not reflective of the way the typical developer works, who consults the Internet to find similar problems and their respective patches when they need debugging assistance. Such a developer needs to understand the posted solution and tailor it to the specific problem they are facing. Rather than focusing on one process, our work focuses on the entire debugging pipeline. We achieve this by first building a dataset of patches. Given previous code, edit position, and some description of the patch, our chosen to ask is to discover what has been done in a similar context before. Once that is determined, we want to input that in a model and generate edits that are similar that may or may not be present in the codebase.

We use MODIT \cite{chakraborty2021multi}, a multi-modal code engine based on the Neural Machine Translator (NMT), to generate patches that are similar to what is inputted. To automatically create modifications with NMT models, MODIT \cite{chakraborty2021multi} uses three modalities of information: edit location, edit code context, and commit messages together as a surrogate for developers' suggestions in natural language. In REDCODER\cite{redcoder}, we saw that including similar code as input to model helped in code generation. We bring the same functionality here by feeding similar patches to MODIT \cite{chakraborty2021multi} as the fourth modality. Our hypothesis is that the patch generation
performance should improve as was seen in the case of REDCODER \cite{redcoder}.

While code generation creates from scratch, editing modifies one part of what already exists. Our study deals with patches, which is more closely related to editing than generating a patch from scratch. We \emph{edit} the buggy line rather than \emph{generate} the buggy line from scratch for patches because we are trying to mimic thought process of a software engineer.

CoditT5 \cite{zhang2022coditt5} generates an edit plan to be applied to the buggy line to generate patches. As the researchers of CoditT5 \cite{zhang2022coditt5} mention, the edit pre-training objective does not help with generation. They use CodeT5 \cite{wang2021codet5} and CoditT5 \cite{zhang2022coditt5} together to generate the best alternatives for patches. We use MODIT \cite{chakraborty2021multi} to generate the patch, which CoditT5 \cite{zhang2022coditt5} further modifies for the problem we are trying to solve.

We summarize our main contributions as follows:
\begin{itemize}[noitemsep, topsep=1pt]
\item To our knowledge, this is the first tool that integrates information retrieval, code generation, and code editing in one pipeline.
\item In addition to CoditT5 \cite{zhang2022coditt5}, we also use another edit-based Transformer model, the Levenshtein Transformer, in a code-based setting.
\item Improvements

\end{itemize}


==> body/2.background.back.tex <==
\section{Background}

An evolving set of technologies called Automated Program Repair allows software systems to automatically fix coding bugs. As a study area, APR focuses on a family of methods that creates source code-level patches for bugs, similar to the patches that programmers create when fixing bugs in their own work or in response to the bug reports they receive. Thus, at a high level, an automated repair technique takes a program and some proof that the program has a defect as input and outputs a patch to remedy the coding bug in the source code, preferably without adversely affecting other proper functionality.

\subsection{Search}

% Automatic bug repair is primarily a search issue with the objective of identifying a collection of software edits that fix a specific error without creating more or changing previously acceptable behavior. 

Search-based APR techniques comb through all permutations of possible patches to find the correct one.
Previous work \cite{jiang2018shaping} indicates that existing patches and similar source code may help to identify the correct patch.
Therefore, similar to the definition of search-based APR, the 
goal of patch search is to find the most relevant patch from a search base, which may help to synthesize the correct patch.

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.33\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/encoder-decoder.pdf}
         \caption{Encoder-decoder}
         \label{fig:encoder-decoder}
     \end{subfigure}
     ~~
     \begin{subfigure}[b]{0.33\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/decoder-only.pdf}
         \caption{Decoder only}
         \label{fig:decoder-only}
     \end{subfigure}
     ~~
     \begin{subfigure}[b]{0.33\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/levtransformer.pdf}
         \caption{Levenshtein Transformer}
         \label{fig:lev-transformer}
     \end{subfigure}
        \caption{Different Types of Transformer-based Generative More  and Levenshtein Transformer}
        \label{fig:three graphs}
\end{figure*}

\section{Background: Code Generation Models}
% \subsubsection{Transformer}

% \subsubsection{Encoder-Decoder}
% \subsubsection{Decoder-Only}
% Neural machine translation is a technique for changing one input sequence into another output sequence using neural networks. Many previous works have modeled the the task of program repair with NMT in an autoregressive manner, which means the decoder generates an output token by reasoning the input sequence and the previous output tokens generated. However, there is a chance that the model may generate a wrong token in a certain position which may make the whole sequence syntactically incorrect.
In recent years, Machine Learning-based Code Generation has gained significant attention, where code is generated from a Natural Language (NL) description or code context. 
Different types of Sequence-to-Sequence ($S2S$ or $seq2seq$) models play a significant role in achieving this success~\cite{pradel2021neural, ding2020patching}.
At a high level, input to an $S2S$ model is a sequence of tokens ($X = x_1, x_2, ..., x_n$), and the output is a token sequence ($Y = y_1, y_2, ..., y_m)$, where  the model learns conditional probability distribution $P(Y|X)$. 

RNN and LSTM-based models~\cite{hochreiter1997long} once held a dominant role in code generation~\cite{chen2019sequencer, chakraborty2020codit, 
nam2022predictive,yin2018learning}. At a high level, these models take a sentence token-by-token in a sequential manner and try to predict the next token depending on the immediately preceding tokens in the sequence. Thus, these models largely depend on the tokens in close vicinity and tend to suffer from not capturing the long-range dependencies.
% with previous tokens (words). 

\subsection{Transformer for Code Generation}

% However, these models typically suffer from long-range dependency issues as they primarily depend on the depend on latest words (and their hidden states) capturing the dependencies with previous tokens (words). 
% which are gradually replaced by Transformer\cite{vaswani2017attention} in recent years.  
% RNN/LSTM-based models take a sentence word by word in a sequential way.
% Thus, these models typically suffer from long-range dependency issues because 
% they depend on the last hidden state capturing the dependencies with previous tokens (words). 
%In recent years,  RNN/LSTM-based models are gradually replaced by Transformers\cite{vaswani2017attention}. 

In recent years, Transformer-based models~\cite{vaswani2017attention} have outperformed alternative architectures for code generation due to the introduction of the self-attention mechanism.
Conceptually, transformers process the entire input token sequence holistically, processing the sequence as a complete graph \footnote{\href{https://en.wikipedia.org/wiki/Complete_graph}} --- each token is a vertex in the graph, and an edge connecting two vertices represents the \enquote{attention} between the corresponding tokens. The attention tries to represent how important that edge is while making the final predictions.
Depending on the task, the model learns the attention weights during the training process. Transformer also encodes the related position of each token in the input sequence  (positional encoding). 

The attention mechanism and positional encoding allow the  Transformer to catch more long-range dependencies. Also, processing the entire input allows more parallelization and a significant speedup during training. With such success of Transformers, many previous works \cite{chen2019sequencer,tufano2019learning,tufano2018empirical,chakraborty2021multi,jiang2021cure,nijkamp2022codegen} have leveraged 
NMT to address code generation problems (e.g. patching, code editing and program repair) in SE community and many recent works \cite{jiang2023knod,xia2022less,chakraborty2020codit} have started to use Transformer model~\rayb{make sure we only use transformer here.}. Transformer-based code generation models roughly fall into two categories: encoder-decoder and decoder-only.


%As opposed to token-by-token processing of RNN/LSTM, Transformer processes the entire input token sequence at once. This allows more parallelization and a significant speedup in training time. 
%can significantly reduce the time needed for training. 
%Moreover, with the introduction of the self-attention mechanism, Transformers are able to capture relevant tokens that are far away from each other in the sequence. Positional encoding further assigns extra vectors to tokens so that the model can identify their relevant positions.
% and positional encoding are also introduced into Transformer~\rayb{explain in one line each what they are}.
% The former one let Transformer being capable of detecting even subtle relevance between tokens that are far away from each other in the sequence.
% The latter one assigns extra vectors to tokens so that the model can identify
% their relevant positions. 
%All these techniques allow Transformer to catch more token-wise relationship information and minimize the %there is basically no 
%risk of forgetting any token in the sequence.

% Moreover, self-attention and positional encoding are also introduced into Transformer~\rayb{explain in one line each what they are}.
% The former one let Transformer being capable of detecting even subtle relevance between tokens that are far away from each other in the sequence.
% The latter one assigns extra vectors to tokens so that the model can identify
% their relevant positions. All these techniques allows Transformer to catch more token-wise relationship and minimize the %there is basically no 
% risk to lose or forget any token in the sequence.



\textbf{Encoder-decoder}. As is shown in Figure \ref{fig:encoder-decoder}, a encoder-decoder model has both a bidirectional Transformer encoder and an autoregressive Transformer decoder. The encoder is trained to extract the feature from the input sequence. 
The decoder always generates the next token by reasoning the feature extracted by the Transformer encoder and previously generated tokens.
In other words, the encoder-decoder model is designed to understand and generate code simultaneously.
PLBART \cite{ahmad2021unified} and NatGen~\cite{chakraborty2022natgen} are  typical encoder-decoder models trained with denoising pretraining. MODIT\cite{chakraborty2021multi} fine-tunes PLBART for code editing task and discusses the impact of different modalities in the input.
CodeT5\cite{wang2021codet5} is an identifier-aware unified pretrained encoder-decoder model, and CoditT5 \cite{zhang2022coditt5} presents a pretrained model customized for editing task using the same architecture as CodeT5. 
%Unlike Modit, the output of CoditT5 is in the format of  \emph{Edit Plan} <s> \emph{patch}.

In fact, some encoder-only Transformer models can be integrated into the encoder-decoder model. For example, \cite{chakraborty2021multi} combined CodeBERT\cite{feng2020codebert} and GraphCodeBERT \cite{guo2020graphcodebert} with a Transformer decoder trained from scratch for code editing.

\textbf{Decoder-only}. Decoder-only models only have an autoregressive Transformer decoder, which is shown in Figure \ref{fig:decoder-only}.
Since there is no encoder, decoder-only is a 
\enquote{generate only} architecture. 
\cite{jiang2021cure} shows the effectiveness 
of GPT for the task of source code patching.
Other representative decoder-only code generation models include OpenAI's Codex\cite{chen2021evaluating} and CodeGen \cite{nijkamp2022codegen}. Decoder-only models are suitable for open-ended code generation, where a prompt describing the functionality is passed to the model.

% which 
%  is able to 
% process the entire input sequence all at once while RNN-based models are limited by memory issues from 
% sequential processing. Furthermore the parallel computation mechanism gives Transformer a 
% higher efficiency. 

\subsection{Levenshtein Transformer}
Different from Transformers that generate the target from scratch, Levenshtein Transformers \cite{gu2019levenshtein} take account of the potential huge overlap between the source sequence and the target sequence and use basic operations \emph{insertion} and \emph{deletion} to implement sequence transformation. The Levenshtein Transformer can be very versatile, proving its flexibility on refinement tasks (e.g. automatic post-editing) as well as machine translation.

We compare the vanilla Transformer and Levenshtein Transformer in Figure\ref{fig:encoder-decoder} and Figure \ref{fig:lev-transformer}. 
They share the same encoder and decoder blocks. The one difference is that the vanilla Transformer devises linear layer and softmax upon stacks of decoder layers to predict next token, while the Levenshtein Transformer uses three additional classifiers to apply edit operations.

The output of the last Transformer decoder block is denoted as 
$h=\{ h_0, h_1, \cdots, h_n \}$ and is passed to following classifiers:

\begin{enumerate}
  \item Deletion Classifier:
  For each token in the sequence, the deletion classifier predicts whether it should be deleted(1) or kept(0).
  \begin{equation}
      \pi_\theta^{\mathrm{del}}(h_i) = softmax(W_{del}h_i)
  \end{equation}
   Where $W_{del}$ is the weight matrix of the deletion classifier.
  \item Placeholder Classifier: predicts how many \emph{place holders} should be inserted between any consecutive token pairs in the whole sequence.
  \begin{equation}
      \pi_\theta^{\mathrm{plh}}(<h_i, h_{i+1}>) = softmax(W_{plh}\cdot concat(h_i, h_{i+1}))
  \end{equation}
  Where $W_plh$ is the weight matrix of the placeholder classifier.
  \item Insertion Classifier: for each placeholder we inserted in the last step, the insertion classifier predicts which token should be actually inserted in this position: 
   \begin{equation}
      \pi_\theta^{\mathrm{ins}}(h_i) = softmax(W_{ins}h_i)
  \end{equation}
  Where $W_{ins}$ is the weight matrix of the insertion classifier.
\end{enumerate}

\subsection{Patch Editing}

The editing approach has recently become a prominent alternative to $seq2seq$ generation for modeling
code fixing and code changing. 
These tasks share a common trait: there is possibly a 
huge overlap between the source sequence and the target sequence.
In contrast, for the bug fixing and code editing tasks, 
generation model generate the patch from scratch token by token.
In this case, the editing model exhibits its strength
in understanding the essence of program defects or code changes.

% \subsection {Research Questions}

% Our hypothesis is that creating an edit pipeline will help us fix more software bugs. This leads to several research questions.

% \newlist{questions}{enumerate}{2}
% \setlist[questions,1]{label=RQ\arabic*.,ref=RQ\arabic*}
% \setlist[questions,2]{label=(\alph*),ref=\thequestionsi(\alph*)}

% \begin{questions}

%     \item What is the overall effectiveness of \tool in editing code? \\
    
%     Different from many previous works, which only focus on patch search or generating patches, we integrate patch search, patch generation and patch editing into one pipeline. \\
%     We observe that compared to generation model baselines \cite{ahmad2021unified, chakraborty2022natgen, zhang2022coditt5}, our overall pipeline
%     can effectively improve the number of successful edits.
%     % To have a better understanding on the effectiveness of our pipeline, we have to further investigate the effectiveness of every component. 
%     To explore the ability of \tool, we further evaluate it on a special case 
%     of code editing: bug fixing.
%     \\
    
%     \item What is the overall effectiveness of \tool in fixing programming bugs?
%     After 
    
%     \item Does patch search help to repair code? \\
    
%     Our hypothesis is that the generated model can always benefit from the extra information provided by retrieved patches. In our study, we construct different queries. Experiment results indicate that different types of retrieved patches can always improve the exact match.\\
%     With the effectiveness of patch search well explored, we further compare our editing model (Levenshtein Transformer) with vanilla Transformer to understand 
%     why it is capable of editing patches. \\
    
%     \item What is the characteristic of the editing model? \\
    
%     Unlike an autoregressive Transformer which generates target sequence token by token, non-autoregressive Levenshtein Transformer generates the target sequence by applying editing operations on the source sequence. In our study,
%     we train and test these two models on the same dataset and compare the correct patches they produced. Experiment results indicate that Levenshtein Transformer is good at fixing 'small bugs', which shows its potential of performing additional editing on patches. \\
    
% \end{questions}



==> body/3b.program_repair.bck.tex <==
\subsection{Generation Model}
% \subsubsection{Pre-trained Weights}
% We fine-tune our generating model on three pre-trained model: PLBART \cite{ahmad2021unified}, CoditT5 \cite{zhang2022coditt5} and NatGen \cite{chakraborty2022natgen}. For all the three pre-trained models,
% the inputs are in the format of ( buggy line <s> context ) or ( buggy line <s> retrieved patches <s> context ). The output of CoditT5 is ( edit plan <s> fixed code ) while others' are fixed code.

\subsubsection{Fine-tuning pre-trained language models}
At the generating stage, we choose the Transformer Encoder-Decoder \cite{vaswani2017attention} as the basic model.
The input of the Transformer Encoder-Decoder model is a sequence of sub-tokens: $ X=\{x_1, x_2, \cdots, x_n\}$.
As shown in Figure \ref{fig:transformer_arch}-(a), the encoder \cite{vaswani2017attention} is composed of several layers, and each layer has two sub-layers: a multi-head self-attention mechanism and a fully connected feed forward
network. Besides, each sub-layer is followed by layer normalization, which means the output of a sub-layer is: $layerNorm(X+subLayer(X))$ 

Similar to the encoder, the decoder (Figure \ref{fig:transformer_arch}-(b)) is also composed of a stack of layers, but each of them has three sub-layers: a masked multi-head self-attention, a cross attention, and a feed-forward network. Masked multi-head self-attention is very similar to the multi-head self-attention in the encoder, but it also receives masks as input so that the attention mechanism does not use the information from hidden/masked positions. The cross attention is another multi-head attention mechanism that calculates the attention weights between the output of the encoder and the input of decoder. The feed-forward network is exactly the same as the one in the encoder.

During the testing/inference stage, the Transformer Encoder-Decoder will repeat the following steps: (1) take the input sequence as the input of the encoder, take the (sub-)tokens that have been generated as the input of the decoder;
(2) compute the probabilities of the next (sub)token;
(3) pick the next (sub)token with beam search. For PLBART \cite{ahmad2021unified}, MODIT \cite{chakraborty2021multi}, and 
NatGen \cite{chakraborty2022natgen}, the target sequence (the sequence we generate) is expected
to be the fixed code; thus, no more post-processing is needed.
However, CoditT5 \cite{zhang2022coditt5} needs further post-processing because its target sequence is in the following format: \emph{Edit Operations} <s> \emph{fixed code}.
\subsubsection{Evaluating large language model(LLM) in the zero-shot manner}
In order to validate the generalization ability of \tool
we directly use the OpenAI's Codex\cite{chen2021evaluating} in a zero-shot setting. Following many previous works \cite{prenner2021automatic, joshi2022repair, fan2022improving}, we design a prompt as the input of Codex, which is a combination of code and natural language.
As is shown in Figure \ref{fig:prompt}, we place a 
comment in the starting line that describes the task
that Codex is expected to carry out: \enquote{fix the bug in the following method}.
The task description is followed by the buggy code, and the location of the buggy line is notified with another comment: \fbox{\mbox{ /// buggy line is here}}.
After the buggy line, we provide Codex with the retrieved patch using another comment. Apart from that, to guide the model focus on 
the repair of the buggy line, the prompt also includes the context before the buggy line which 
starts with a comment: \fbox{\mbox{ /// change the buggy line to fix the bug:}}.

After incorporating a buggy code snippet with the prompt and feeding it to Codex, we always 
take the first line in the code generated by Codex as the patch.

\begin{figure}[h]
    \includegraphics[width=\linewidth]{figures/prompt.pdf}\par
    \centering
    \caption{An example of the prompt (Codec-17). The prompt 
    includes the buggy code (green lines), buggy line (red 
    line), retrieved patch (yellow line) and the context before the buggy line(pink lines). }
    \label{fig:prompt}
\end{figure}

\subsection{Editing Model}
\begin{figure}[h]
    \includegraphics[width=\linewidth]{figures/TRANSFORMER.jpg}\par
    \centering
    \caption{Transformer and Levenshtein Transformer}
    \label{fig:transformer_arch}
\end{figure}

At the editing stage, we further edit the generated patches.
%which cannot pass the test suit. 
The editing model in an edit-base Levenshtein Transformer \cite{gu2019levenshtein} that edits patches via deletion and insertion
operations.

\subsubsection{Model Architecture}

Unlike the typical autoregressive Transformer decoder that has only one prediction head to predict the next output word,
Levenshtein Transformer decoder has three classifiers: 
an Insertion Classifier, Deletion Classifier and Placeholder Classifier.
The difference between a standard Transformer decoder and a Levenshtein Transformer decoder is shown in Figure \ref{fig:transformer_arch}.
The output of the last Transformer decoder block is denoted as 
$h=\{ h_0, h_1, \cdots, h_n \}$ and is passed to the three classifiers:

\begin{enumerate}
  \item Deletion Classifier:
  for each token in he sequence, deletion classifier predicts whether it should be deleted(1) or kept(0).
  \begin{equation}
      \pi_\theta^{\mathrm{del}}(h_i) = softmax(W_{del}h_i)
  \end{equation}
Where $W_{del}$ is the weight matrix of the deletion classifier.
  \item Placeholder Classifier: predicts how many 'place holders' should be inserted between any consecutive token pairs in the whole sequence.
  \begin{equation}
      \pi_\theta^{\mathrm{plh}}(<h_i, h_{i+1}>) = softmax(W_{plh}\cdot concat(h_i, h_{i+1}))
  \end{equation}
  Where $W_plh$ is the weight matrix of the placeholder classifier.
  \item Insertion Classifier: for each placeholder we inserted in the last step, the insertion classifier predicts which token should be actually inserted in this position: 
   \begin{equation}
      \pi_\theta^{\mathrm{ins}}(h_i) = softmax(W_{ins}h_i)
  \end{equation}
  Where $W_{ins}$ is the weight matrix of the insertion classifier.
\end{enumerate}

% \subsubsection{Model Training}
% Following Gu et al. \cite{gu2019levenshtein}, we adopt imitation learning to train our model.
\subsubsection{Patch Editing}
At the inference stage, we use patches synthesized by the generating model ($Y$) as the initial input of the decoder. Then we perform the following edit operations:
\begin{itemize}
    \item Make deletion prediction with $ \pi_\theta^{\mathrm{del}}$ on the top of $Y$.The output is 
    denoted as $Y'$.
    \item Insert placeholder is before every token in the deleted sequence $Y'$ with $\pi_\theta^{\mathrm{plh}}$, the output is denoted as $Y''$.
    \item Insert tokens into placeholders with $ \pi_\theta^{\mathrm{ins}}$ and output $Y'''$. 
\end{itemize}

Different from other code editing model like CoditT5 \cite{zhang2022coditt5} and Plur \cite{chen2021plur}, which generate edit plan or other output representing code edit, our model directly edits the code in the process of generating the output.

\subsection{Patch / Edit Validation}
During the inference stage, we run \tool on Defects4j \cite{just2014defects4j}, a framework with faulty and fixed program versions 
and corresponding test suite. Following previous work \cite{lutellier2020coconut}, we call patches
synthesized by our generating/editing model \enquote{candidate patches}.
After validating the candidate patches with the corresponding test suit, 
they can be further classified into following categories:
\begin{itemize}
\item \textbf{Correct patches:} Exactly the same as the patches provided by Defects4j.
\item \textbf{Plausible patches:} Can pass the test suite, but cannot guarantee if they are correct patches. 
% \item \textbf{Compilable patches:} After applying candidate patches the project can be compiled.
\end{itemize}


==> body/5c.results_and_analysis_ablation.tex <==
%\subsection{RQ3. Ablation study: what's the contribution of Search and Edit?}
\subsection{RQ2. Contributions of Search and Edit}

\subsubsection{Motivation}
To investigate the contribution of each step (search, generation, and modify), we present an ablation study for each step of \tool.
%, i.e., how much each component contributes to the final results. 

\subsubsection{Experimental Setup}
For both the task of code editing and program repair, we follow the basic setup of RQ.1. % and RQ.2. 
In this section, we evaluate the following variants of \tool:
\begin{itemize}[leftmargin=*]
    \item \textbf{Search}: Evaluate the edits/patches produced by the search step only. %edit/patch search.
    \item \textbf{Search + Generate}: Combine the retrieved patch with the original input, %(buggy line, context, and commit message (if applicable), 
    pass the combined input to a generative model, and evaluate the output.
    \item \textbf{Search + Generate + Modify}: Further modify  the output of \\ Search\-+Generate with the modification  model.
\end{itemize}

We further investigate the $top\ 1$ and $top\ 5$ patch generation in each setting.
% impact of the number of retrieved edits on the final results. 
% For the code editing task, we present the results based on top-1 and top-5 retrieved edits. 
% %For program repair task,  we use top-1, top-5, and top-25 retrieved edits. 
% Note that, for each of these settings, we only consider the top-1 output of the generative model, as code generation is not our primary contribution. 
% However, as shown in~\Cref{table:2}, the overall findings hold for top-k generation as well.
%regarding the generation model, we only present 
%the top-1 output for experiments on code editing~\rayb{why?}.

\begin{figure}[h]
     \centering
     \begin{subfigure}[]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ablation_1.png}
         \caption{Ablation study on \sdata }
         \label{fig:ablation_d4j1}
     \end{subfigure}
     \begin{subfigure}[]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/ablation_2.png}
         \caption{Ablation study on \mdata}
         \label{fig:ablation_d4j2}
     \end{subfigure}
    \caption{Ablation Study on \sdata and \mdata}
    \label{fig:ablation_b2f}
\end{figure}

\subsubsection{Results}
\textbf{Code Editing.} Figure \ref{fig:ablation_b2f} shows the effectiveness of components of \tool : for all the three
off-the-shelf code generation models, adding search can improve the patch generation, and modifying the generated patch can further improve the performance. For example, on \sdata retrieved edits can improve the $top\ 1$ exact match of PLBART \cite{ahmad2021unified} by $3.97\%$, and the modifying step further 
improves it with another $1.81\%$. Such a improvement can also be found on \mdata. For instance, retrieved patches improve generate-only PLBART \cite{ahmad2021unified} from 36.51\% to 37.57\% and the modification model further boost up accuracy with another 2.24\%.    

% Another observation is that taking more retrieved 
% edits can also boost the exact match. Compared with only taking the top-1, taking top-5 means we are 
% able to search $0.96\%$ more correct edits from the training set. More retrieved edits can also improve
% the performance of the generation model. For example, it can improve CoditT5 by $6.14\%$.

% \begin{figure*}[h]
%      \centering
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/ablation_3.png}
%          \caption{\textbf{Defect4j$_{1.2}$}}
%          \label{fig:ablation_d4j1}
%      \end{subfigure}
%      ~
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/ablation_4.png}
%          \caption{\textbf{Defect4j$_{2.0}$}}
%          \label{fig:ablation_d4j2}
%      \end{subfigure}
%         \caption{Ablation study on Defects4J }
%         \label{fig:ablation_d4j}
% \end{figure*}

% \textbf{Program Repair.} 
% In the ablation study on Defects4J, we fix the number of retrieved
% patches to 25, and set k to 1, 10, 50. In other words, Codex generates
% 25, 250 and 1250 with respect to different top-k. \yogesh{I dont think we mentioned Codex in our experimental setup. We need to mention it}
% Figure \ref{fig:ablation_d4j} can further prove the effectiveness 
% of search and edit. Similar to what 
% we find out in Figure \ref{fig:ablation_b2f}, increasing to number of
% top-k in the generation model (Codex) can always lead to more correct fixes.
% According to Figure \ref{fig:ablation_b2f} and Figure \ref{fig:ablation_d4j},
% if we can increase the number of patches produced by the pipeline to match the
% larger number (e.g. 5,000) used by other tools (e.g. AlphaRepair), a higher number
% of correct fixes can be expected.


\begin{answerbox}
\textbf{Result 2}: Both the search and edit are essential for \tool to synthesize correct patches. With respect to $top\ 1$ accuracy, search brings up to 3.97\% more correct patches and edit can brings up to 2.24\% more successful patches.
\end{answerbox}






==> body/5d.results_and_analysis_levenshtein_old.tex <==
\subsection{Characteristic of Editing Model}
% \begin{questionbox}
% \textbf{RQ.3 What is the characteristic of the editing model?}
% \end{questionbox}
\subsubsection{Experimental Setup}
To analyze the characteristics of the editing model in our pipeline, we compare the Levenshtein Transformer with 
standard Transformer model.
Similar to \emph{RQ.2}, we train both the Transformer models % and Levenshtein Transformer model 
from scratch
on the same Bug2Fix \cite{chakraborty2021multi} dataset.
After that we further compare the correct edits produced by these two models using the following evaluation metrics:
edit distance, tree editing distance, and the average number of new identifiers introduced.
In our experiment, the input is in the format of \emph{buggy line} <s> \emph{context} <s> \emph{commit message}, and the output is the fixed code.



\begin{figure}
     \centering
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/VENN1.jpeg}
         \caption{Bug2Fix\_small}
         \label{fig:VENN@small}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/VENN2.jpeg}
         \caption{Bug2Fix\_medium}
         \label{fig:VENN@medium}
     \end{subfigure}
        \caption{Analysis of the correct edit produced by Transformer and Levenshtein Transformer}
        \label{fig:VENN}
\end{figure}


\subsubsection{Results}
As is shown in Figure \ref{fig:VENN@small}, we can see that LevT and Transformer perform 966 and 909 correct edits respectively on test set of Bug2Fix\_small. Among the 966 correct edits, 468 of them are only performed by LevT.
Among the 909 correct edits performed by Transformer, 411 of them are only performed by Transformer. On Bug2Fix\_medium we can find 272 
overlapped correct edits shared by LevT and Transformer model. They can perform the other 284 correct edits and 343 correct edits respectively.

To understand the characteristics of the LevT, we calculate the averaged edit distance of edits performed by LevT and Transformer in different areas
in Figure \ref{fig:VENN}, which is reported in Table \ref{Table@Edit_Dis}. In area A, where LevT can perform successful edits, the averaged edit distance of successful edits is 6.147, which is obviously lower than the averaged 
edit distance of those in area C (8.644), where Transformer can perform successful edits.
Similar circumstances also happen in areas D and F.
In area D, the correct edits performed by LevT have a smaller average edit distance than the incorrect counterparts of Transformer. In area F, the correct edits applied by Transformer have a relatively larger averaged 
edit distance than those performed by LevT.

To further evaluate the finding we got from Table \ref{Table@Edit_Dis}, we also calculate the tree edit distance of edits in different areas in Figure \ref{fig:VENN}.
Table \ref{Table@Edit_Tree_Dis} shows us that the correct edits performed by LevT always have smaller tree edit distance compared to the correct edits applied by Transformer.

\begin{table}[]
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Area} & \textbf{\begin{tabular}[c]{@{}c@{}}Levenshtein \\ Transformer\end{tabular}} & \textbf{Transformer} & \textbf{P-Value}                                       & \textbf{\begin{tabular}[c]{@{}c@{}}Mannwhitney U \\ P-Value\end{tabular}} \\ \hline
\textbf{A}    & 6.157                                                                       & 7.599                & 0.000499                                               & 0.00335                                                                   \\ \hline
\textbf{B}    & 6.488                                                                       & 6.488                & -                                                      & -                                                                         \\ \hline
\textbf{C}    & 6.908                                                                       & 8.664                & 0.00076                                                & 0.00022                                                                   \\ \hline
\textbf{D}    & 6.954                                                                       & 10.439               & $8.846 \times 10^{-7}$ & $4.552\times 10^{-5} $                    \\ \hline
\textbf{E}    & 4.956                                                                       & 4.956                & -                                                      & -                                                                         \\ \hline
\textbf{F}    & 5.654                                                                       & 8.112                & 0.013                                                  & 0.0039                                                                    \\ \hline
\end{tabular}
}
\caption{Averaged Edit Distance of Edits performed by Levenshtein Transformer and Transformer in Different Areas in Figure \ref{fig:VENN}}
\label{Table@Edit_Dis}
\end{table}


\begin{table}[]
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Area} & \textbf{\begin{tabular}[c]{@{}c@{}}Levenshtein \\ Transformer\end{tabular}} & \textbf{Transformer} & \textbf{P-Value} & \textbf{\begin{tabular}[c]{@{}c@{}}Mannwhitney U \\ P-Value\end{tabular}} \\ \hline
\textbf{A}    & 12.322                                                                      & 15.872               & 0.000302         & 0.07857                                                                   \\ \hline
\textbf{B}    & 14.141                                                                      & 14.141               & -                & -                                                                         \\ \hline
\textbf{C}    & 15.136                                                                      & 18.146               & 0.011962         & 0.00521                                                                   \\ \hline
\textbf{D}    & 14.727                                                                      & 22.101               &   $3.870 \times 10^{-6}$               & 0.00682                                                                   \\ \hline
\textbf{E}    & 11.272                                                                      & 11.272               & -                & -                                                                         \\ \hline
\textbf{F}    & 12.648                                                                      & 18.844               & 0.02286          & 0.03930                                                                   \\ \hline
\end{tabular}
}
\caption{Averaged Tree Edit Distance of Edits performed by Levenshtein Transformer and Transformer in Different Areas in Figure \ref{fig:VENN}}
\label{Table@Edit_Tree_Dis}
\end{table}


\begin{table}[]
\scalebox{0.85}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Area} & \textbf{\begin{tabular}[c]{@{}c@{}}Levenshtein \\ Transformer\end{tabular}} & \textbf{Transformer} & \textbf{P-Value} & \textbf{\begin{tabular}[c]{@{}c@{}}Mannwhitney U \\ P-Value\end{tabular}} \\ \hline
\textbf{A}    & 0.355                                                                       & 1.400                & $3.740\times 10^{-21}$        & $2.096 \times 10^{-24}$                                                                 \\ \hline
\textbf{B}    & 0.489                                                                       & 0.489                & -                & -                                                                         \\ \hline
\textbf{C}    & 0.336                                                                       & 0.910                & $2.310 \times 10^{-13} $        & $4.680 \times 10^{-13}$                                                                 \\ \hline
\textbf{D}    & 0.278                                                                       & 1.045                & $1.435 \times 10^{-24}$        & $6.052 \times 10^{-33}$                                                                 \\ \hline
\textbf{E}    & 0.327                                                                       & 0.327                & -                & -                                                                         \\ \hline
\textbf{F}    & 0.255                                                                       & 0.839                & $8.323 \times 10^{-21}$        & $2.231 \times 10^{-21}$                                                                 \\ \hline
\end{tabular}
}
\caption{Averaged Number of New Identifiers Introduced of Edits performed by Levenshtein Transformer and Transformer in Different Areas in Figure \ref{fig:VENN}}
\label{Table@New_Identi}
\end{table}

In Table \ref{Table@New_Identi}, we calculate the averaged number of new identifiers introduced to the edited code. Results indicate that in areas A and D, the correct edits performed by LevT are always introducing much fewer new identifiers compared to the wrong edits produced by Transformer. Like what we have found in Table \ref{Table@Edit_Dis} and Table \ref{Table@Edit_Tree_Dis}, similar things happen in Area C and Area F.

% \mybox{
% \textbf{Result 3}: Compared to Transformer, Levenshtein Transformer always produce edits with smaller 
% }

% \begin{answerbox}
% \textbf{Result 3}: Compared to Transformer, Levenshtein Transformer always produce edits with smaller (tree) edit distance and fewer identifiers introduced, 
% which indicates that Levenshtein prone to fix 'small bugs'.
% \end{answerbox}

==> body/5e.results_and_analysis_patch_search_old.tex <==

\subsection{RQ4. Insights on Search.}
% \begin{questionbox}
% \textbf{RQ 1. Does patch search help to repair code?}
% \end{questionbox}
\subsubsection{Experimental Setup}
Code Embeddings were generated using PLBART \cite{ahmad2021unified} and TF-IDF. Sections 3.1.2 and 3.1.3 were performed with the k values 1 and 5. All experiments were done on the $B2F_{s}$ dataset.
Pre-trained PLBART \cite{ahmad2021unified} is not fine-tuned on the dataset to get code embeddings.

The datasets used for similarity measurement were \texttt{prev\textunderscore code} and \texttt{fixed\textunderscore only}. 
The latter was used to evaluate and confirm that the PLBART \cite{ahmad2021unified} embeddings were able to capture more semantic and syntactic information as compared to those created with TF-IDF. 

When passing multiple modalities as input to get embeddings, they are formatted as such.
<modality 1> <s> <modality 2>.



\begin{table*}[htbp]
\begin{tabular}{|c|ccc|cccc|}
\hline
\multirow{2}{*}{} &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Retrieved Fixed Code query with \\ (just 1 as query)\end{tabular}}} &
  \multicolumn{4}{c|}{\textbf{Accuracy}} \\ \cline{2-8} 
 &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Buggy \\ Lines\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Context \end{tabular}}} &
  \textbf{Commit} &
  \multicolumn{2}{c|}{\textbf{Small}} &
  \multicolumn{2}{c|}{\textbf{Medium}} \\ \hline
\multirow{8}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Query with \\ individual \\ item \\ (simple Query)\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{-}} &
  \multicolumn{1}{c|}{\textbf{-}} &
  - &
  \multicolumn{1}{c|}{\textbf{29.99}} &
  \multicolumn{1}{c|}{\textbf{\%improve}} &
  \multicolumn{1}{c|}{\textbf{23.02}} &
  \textbf{\% improve} \\ \cline{2-8} 
 &
  \multicolumn{1}{c|}{-} &
  \multicolumn{1}{c|}{-} &
  1 &
  \multicolumn{1}{c|}{31.97} &
  \multicolumn{1}{c|}{6.60\%} &
  \multicolumn{1}{c|}{23.81} &
  3.43\% \\ \cline{2-8} 
 &
  \multicolumn{1}{c|}{-} &
  \multicolumn{1}{c|}{1} &
   &
  \multicolumn{1}{c|}{31.92} &
  \multicolumn{1}{c|}{6.44\%} &
  \multicolumn{1}{c|}{24.49} &
  6.39\% \\ \cline{2-8} 
 &
  \multicolumn{1}{c|}{-} &
  \multicolumn{1}{c|}{1} &
  1 &
  \multicolumn{1}{c|}{33.96} &
  \multicolumn{1}{c|}{13.24\%} &
  \multicolumn{1}{c|}{24.43} &
  6.13\% \\ \cline{2-8} 
 &
  \multicolumn{1}{c|}{1} &
  \multicolumn{1}{c|}{-} &
  - &
  \multicolumn{1}{c|}{31.5} &
  \multicolumn{1}{c|}{5.04\%} &
  \multicolumn{1}{c|}{24.72} &
  7.38\% \\ \cline{2-8} 
 &
  \multicolumn{1}{c|}{1} &
  \multicolumn{1}{c|}{-} &
  1 &
  \multicolumn{1}{c|}{32.82} &
  \multicolumn{1}{c|}{9.44\%} &
  \multicolumn{1}{c|}{25.27} &
  9.77\% \\ \cline{2-8} 
 &
  \multicolumn{1}{c|}{1} &
  \multicolumn{1}{c|}{1} &
  - &
  \multicolumn{1}{c|}{31.85} &
  \multicolumn{1}{c|}{6.20\%} &
  \multicolumn{1}{c|}{25.01} &
  8.64\% \\ \cline{2-8} 
 &
  \multicolumn{1}{c|}{1} &
  \multicolumn{1}{c|}{1} &
  1 &
  \multicolumn{1}{c|}{33.63} &
  \multicolumn{1}{c|}{12.14\%} &
  \multicolumn{1}{c|}{24.33} &
  5.69\% \\ \hline
\end{tabular}
\caption{Patch generation results for $B2F$ dataset with \\ retrieved patches as an additional modality to MODIT.}
\label{table:2}
\end{table*}



\subsubsection{Results}
We plot the normalized Levenshtein distance between the retrieved patches and target patch. 
We calculate the distance for both the top retrieved patch and $top\ 5$ retrieved patches. 
The distance for $top\ 5$ patches is calculated by taking the minimum of the distance.
A patch is said to be good if the number of edits to change it to target patch are low.
The plots are presented in Figure X.
The edit distribution's mode for PLBART \cite{ahmad2021unified} retrieved patches are more shifted towards zero. 
We plot the edit distance for the target data as query to confirm whether PLBART \cite{ahmad2021unified} embeddings are better for retrieval.
We perform statistical test to quantify the difference in the two edit distributions.

\vspace*{.4\baselineskip}  

\begin{tabular}{ |c|c|c|c|}
 \hline
 \centering
 Distribution & \begin{tabular}{@{}c@{}}Z Test \\ Statistic\end{tabular} & P value & \begin{tabular}{@{}c@{}}Wasserstein \\ Distance\end{tabular} \\
\hline

\begin{tabular}{@{}c@{}}Prev(PLBART) - \\ Prev(tf-idf) (k=1)\end{tabular}
  & 3.6533  & 0.0002588 & 0.021475  \\
\hline

\begin{tabular}{@{}c@{}}Fixed(PLBART) - \\ Fixed(tf-idf) (k=1)\end{tabular}  & 28.38849  & 2.80472 & 0.13397 \\
\hline
\end{tabular}

\vspace*{.4\baselineskip} 

\begin{figure}[b]

\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/Fig 1- data=prev_code, k=1, PLBART.png}
    \caption{data=\texttt{prev\textunderscore code}, k=1, model=PLBART}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/Fig 2- data=prev_code, k=5, PLBART .png}
    \caption{data=\texttt{prev\textunderscore code}, k=5, model=PLBART}
\end{subfigure}

\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/Fig 3- data=prev_code, k=1, TF-IDF .png}
    \caption{data=\texttt{prev\textunderscore code}, k=1, model=TF-IDF}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/Fig 4- data=prev_code, k=5, TF-IDF .png}
    \caption{data=\texttt{prev\textunderscore code}, k=5, model=TF-IDF}
\end{subfigure}

\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\linewidth]{figures/Fig 5- data=fixed_only, k=1, PLBART .png}
    \caption{data=\texttt{fixed\textunderscore only}, k=1, model=PLBART}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/Fig 6- data=fixed_only, k=5, PLBART .png}
    \caption{data=\texttt{fixed\textunderscore only}, k=5, model=PLBART}
\end{subfigure}

\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\linewidth]{figures/Fig 7- data=fixed_only, k=1, TF-IDF .png}
    \caption{data=\texttt{fixed\textunderscore only}, k=1, model=TF-IDF}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/Fig 8- data=fixed_only, k=5, TF-IDF .png}
    \caption{data=\texttt{fixed\textunderscore only}, k=5, model=TF-IDF}
\end{subfigure}
\caption{Normalized edit distance experiments}
\end{figure}

Based on the results in table X, we used the PLBART \cite{ahmad2021unified} model with different datasets and various k values to assess the highest yielding results. 
We set PLBART’s tokenizer’s \texttt{src\textunderscore lang} and \texttt{tgt\textunderscore lang} as ‘java’ for all variations except for the \texttt{commit\textunderscore msg} dataset. 
For that, we experimented with both \texttt{src\textunderscore lang} and \texttt{tgt\textunderscore lang} as ‘java’ and  \texttt{en\textunderscore XX} as it contains only natural descriptions.\\
Here are the variations: 
\begin{itemize}[nosep, after=\vspace{0.3\baselineskip}]
\item k = 1, 5
\item Dataset:
\begin{itemize}
\item \texttt{prev\textunderscore code} : \texttt{src\textunderscore lang}=java, \texttt{tgt\textunderscore lang}=java

\item \texttt{buggy\textunderscore only} : \texttt{src\textunderscore lang}=java, \texttt{tgt\textunderscore lang}=java

\item \texttt{commit\textunderscore msg} : \texttt{src\textunderscore lang}=\texttt{en\textunderscore XX}, \texttt{tgt\textunderscore lang}=\texttt{en\textunderscore XX}

\item \texttt{commit\textunderscore msg} : \texttt{src\textunderscore lang}=java, \texttt{tgt\textunderscore lang}=java

\end{itemize}
\end{itemize}

The normalized edit distance for these variations are plotted.
We observe that \texttt{buggy\textunderscore only} is best for retrieving patches as compared to \texttt{prev\textunderscore code} or \texttt{commit\textunderscore msg}.
The edit distribution of patches retrieved using \texttt{commit\textunderscore msg} is poor with a mode of 0.8.
The edit distribution of patches retrieved using \texttt{buggy\textunderscore only} is dense on 0 edit distance.
We also compute the statistical significance of the difference between these two distributions.
All the tests were performed on the ‘small train’ dataset.
\\

\begin{tabular}{ |c|c|c|c|}
\hline
\centering
Distribution & \begin{tabular}{@{}c@{}}Z Test \\ Statistic\end{tabular} & P value & \begin{tabular}{@{}c@{}}Wasserstein \\ Distance\end{tabular} \\
\hline
\begin{tabular}{@{}c@{}}Buggy - Commit\\ (k=1, PLBART)\end{tabular}  & -110.6455  & 0.0 & 0.1636  \\
\hline
\begin{tabular}{@{}c@{}}Buggy - Prev\\ (k=1, PLBART)\end{tabular}  & -49.2569  & 0.0 & 0.0784  \\
\hline
\begin{tabular}{@{}c@{}}Prev - Commit\\ (k=1, PLBART)\end{tabular} & -56.35098  & 0.0 & 0.08517  \\
\hline
\end{tabular}

\vspace*{.3\baselineskip}  

We get a p-value of less than 0.01 in all scenarios so we can say that the difference between 2 means of the distribution is statistically significant.
The results denote that \texttt{buggy\textunderscore only} is more suitable for patch retrieval.
We observe that the normalized edit distance distribution is worst for the dataset ‘\texttt{commit\textunderscore msg}’.
This is surprising as one would expect that the commit message would contain the most amount of information related to the change and fix in the code. 
However, the results did not reflect this assumption. 
We hypothesize that this is due to the noise present in the dataset. 
Many developers write poor commit messages such as ‘minor fix’, ‘small bug fix’ etc., which does not provide the model enough information about what is actually being fixed. 
Because the dataset has a huge distribution of such messages, the code similarity metric fails to retrieve the correct code fixes from the database.

\begin{figure}[H]
    
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/Fig 9- data=buggy_only, k=1, PLBART.png}
        \caption{data=\texttt{buggy\textunderscore only}, k=1, model=PLBART}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/Fig 10- data=buggy_only, k=5, PLBART.png}
        \caption{data=\texttt{buggy\textunderscore only}, k=5, model=PLBART}
    \end{subfigure}
    
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/Fig 11- data=commit_msg, k=1, PLBART, src_lang=’java’, tgt_lang=’java’.png}
        \caption{data=\texttt{commit\textunderscore msg}, k=1, model=PLBART, \texttt{src\textunderscore lang}=java, \texttt{tgt\textunderscore lang}=java}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/Fig 12- data=commit_msg, k=5, PLBART, src_lang=’java’, tgt_lang=’java’.png}
        \caption{data=\texttt{commit\textunderscore msg}, k=5, model=PLBART, \texttt{src\textunderscore lang}=java, \texttt{tgt\textunderscore lang}=java}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/Fig 13- data=buggy_only <s> commit_msg, k=1, PLBART.png}
        \caption{data=\texttt{buggy\textunderscore only} <s> \texttt{commit\textunderscore msg} , k=1, model=PLBART}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/Fig 14- data=buggy_only <s> commit_msg, k=5, PLBART.png}
        \caption{data=\texttt{buggy\textunderscore only} <s> \texttt{commit\textunderscore msg} , k=5, model=PLBART}
    \end{subfigure}
\end{figure}

\begin{figure}[H] \ContinuedFloat
    
    \begin{subfigure}{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/Fig 15- data=commit_msg, k=1, PLBART, src_lang=’en_XX’, tgt_lang=’en_XX’.png}
        \caption{data=\texttt{commit\textunderscore msg}, k=1, model=PLBART, \texttt{src\textunderscore lang}=\texttt{en\textunderscore XX}, \texttt{tgt\textunderscore lang}=\texttt{en\textunderscore XX}}
    \end{subfigure}
    
    \caption{experiments}
\end{figure}

The ‘\texttt{prev\textunderscore code}’ dataset gives better results as compared to ‘\texttt{commit\textunderscore msg}’. 
We obtain the best results for the dataset ‘\texttt{buggy\textunderscore only}’. 
This is expected as ‘\texttt{prev\textunderscore code}’ refers to the whole code and therefore may contain information not related to the bug. 
Since ‘\texttt{buggy\textunderscore only}’ refers to the part of the code where the bug is located and therefore does not contain noise in the data, we get better results.

We also do an analysis to find if there is any correlation between the inputs used for retrieving patches.
We plot the edit distance between retrieved patch and target patch for the train, eval and test datasets (Figures 7,8,9).
For each plot we observe a diagonal line. 
The diagonal line represents a strong correlation between the x and y axis. 
This suggests that we would get similar results irrespective of the input mechanism in those regions. 
We also observe that  ‘\texttt{buggy\textunderscore only}’ retrieval is better and more concentrated in the 0.60-0.80 region whereas ‘\texttt{prev\textunderscore only}’ is more spread out with higher concentration in >0.80 region.

\begin{figure}[h]
\centering
\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/Fig 16- data=buggy_only vs commit_msg, k=1, PLBART, src_lang=’java’, tgt_lang=’java’.png}
    \caption{data=\texttt{commit\textunderscore msg}, k=1, model=PLBART, \texttt{src\textunderscore lang}=\texttt{en\textunderscore XX}, \texttt{tgt\textunderscore lang}=\texttt{en\textunderscore XX}}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/Fig 17- data=buggy_only vs prev_code, k=1, PLBART.png}
    \caption{data=\texttt{commit\textunderscore msg}, k=1, model=PLBART, \texttt{src\textunderscore lang}=\texttt{en\textunderscore XX}, \texttt{tgt\textunderscore lang}=\texttt{en\textunderscore XX}}
\end{subfigure}

\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/Fig 18-data=prev_codevscommit_msg,k=1,PLBART,src_lang=’java’, tgt_lang=’java’.png}
    \caption{data=\texttt{commit\textunderscore msg}, k=1, model=PLBART, \texttt{src\textunderscore lang}=\texttt{en\textunderscore XX}, \texttt{tgt\textunderscore lang}=\texttt{en\textunderscore XX}}
\end{subfigure}
\caption{Results for train}
\end{figure}

\begin{figure}[h]
\centering
\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/fig19.png}
    \caption{data= \texttt{buggy\textunderscore only} vs \texttt{commit\textunderscore msg}, k=1, model=PLBART, \texttt{src\textunderscore lang}=java, \texttt{tgt\textunderscore lang}=java}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/fig20.png}
    \caption{data=\texttt{commit\textunderscore msg}, k=1, model=PLBART, \texttt{src\textunderscore lang}=\texttt{en\textunderscore XX}, \texttt{tgt\textunderscore lang}=\texttt{en\textunderscore XX}}
\end{subfigure}

\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/fig21.png}
    \caption{data=\texttt{commit\textunderscore msg}, k=1, model=PLBART, \texttt{src\textunderscore lang}=\texttt{en\textunderscore XX}, \texttt{tgt\textunderscore lang}=\texttt{en\textunderscore XX}}
\end{subfigure}
\caption{Results for eval}
\end{figure}

\begin{figure}[H]
\centering
\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/fig22.png}
    \caption{data=\texttt{buggy\textunderscore only} vs \texttt{commit\textunderscore msg}, k=1, model=PLBART, \texttt{src\textunderscore lang}=java, \texttt{tgt\textunderscore lang}=java}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/fig23.png}
    \caption{data=\texttt{buggy\textunderscore only} vs \texttt{prev\textunderscore code}, k=1, model=PLBART}
\end{subfigure}

\begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/fig24.png}
    \caption{data=\texttt{prev\textunderscore code} vs \texttt{commit\textunderscore msg}, k=1, model=PLBART, \texttt{src\textunderscore lang}=java, \texttt{tgt\textunderscore lang}=java}
\end{subfigure}
\caption{Results for test}
\end{figure}

An example of the retrieved patch dataset for ‘small eval’ set can be seen in Figure 8.

\begin{figure}
\begin{subfigure}{0.4\textwidth}
\begin{minted}[fontsize=\mintedfsize, escapeinside=||, linenos]{java}
if ( mConstructionFinished ){ 
    throw new java.lang.IllegalStateException( 
        "Construction finished, 
            TransFormula must not be modified." ); 
} else { 
    return mBranchEncoders . addAll ( arg0 ); 
} 
  
\end{minted}
\caption{Fixed Code}
\vspace{10pt}
\label{Fig@OVER@MOTI@CUT}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\begin{minted}[fontsize=\mintedfsize, escapeinside=||, linenos]{java}
if ( mConstructionFinished ){
    return mBranchEncoders . addAll ( arg0 ); 
} else { 
    throw new java.lang.IllegalStateException( 
        "Construction finished, 
            TransFormula must not be modified." ); 
} 
\end{minted}
\caption{Buggy Only}
\vspace{10pt}
\label{Fig@OVER@MOTI@CUT}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\begin{minted}[fontsize=\mintedfsize, escapeinside=||, linenos]{java}
if ( mConstructionFinished ) { 
    throw new java.lang.IllegalStateException ( 
        "Construction finished, 
            TransFormula must not be modified." ) ; 
} else { 
    return mAuxVars . remove ( arg0 ) ; 
}
\end{minted}
\caption{Buggy Fixed}
\vspace{10pt}
\label{Fig@OVER@MOTI@CUT}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\begin{minted}[fontsize=\mintedfsize, escapeinside=||, linenos]{java}
public boolean addBranchEncoders ( 
 final java.util.Collection < ? 
  extends 
   de.uni_freiburg.informatik.ultimate.logic.TermVariable > arg0){ 
      if ( mConstructionFinished ) { 
        return mBranchEncoders . addAll ( arg0 ) ; 
       } else { 
        throw new java.lang.IllegalStateException ( 
          "Construction finished, 
            TransFormula must not be modified.") ; 
       }
    }
\end{minted}
\caption{Prev Code}
\vspace{10pt}
\label{Fig@OVER@MOTI@CUT}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
\begin{minted}[fontsize=\mintedfsize, escapeinside=||, linenos]{java}
if ( mConstructionFinished ) { 
    throw new java.lang.IllegalStateException ( 
        "Construction finished, 
            TransFormula must not be modified." ) ; 
} else { 
    mInVars . putAll ( m ) ; 
}
\end{minted}
\caption{Prev Fixed}
\vspace{10pt}
\label{Fig@OVER@MOTI@CUT}
\end{subfigure}
\caption{An example from small eval.}
\end{figure}

The ‘\texttt{fixed\textunderscore code}’ is the target patch.
The ‘\texttt{buggy\textunderscore only}’ column is the patch retrieved using \texttt{buggy\textunderscore only} as query.
The ‘\texttt{prev\textunderscore code}’ column is the patch retrieved using \texttt{prev\textunderscore code} as query.
Our method was successfully able to retrieve high quality patches for both short and long code snippets as query.
For the third and fourth example, we observe that although the edit distance for the patch retrieved using \texttt{buggy\textunderscore only} is ~ 0.7, the patch contains partial information.
The \texttt{prev\textunderscore code} performs considerably poorer and retrieves random patches.

\subsubsection{Code Generation}
Table 2 shows the results on patch generation for $B2F$ dataset with retrieved patches as an additional modality to MODIT \cite{chakraborty2021multi}.
Training the model on an additional modality allows to increase its performance for all variations.
The results show that the patches obtained with \texttt{commit\textunderscore msg} as query to Patch Retrieval component gives a better performance as compared to \texttt{buggy\textunderscore only} and \texttt{prev\textunderscore code}.
This is not expected as the figure X shows that the edit distribution for \texttt{commit\textunderscore msg} was worst as compared to others.
We hypothesize that as the patch retrieved using \texttt{buggy\textunderscore only} is similar to target patch, the model learns to focus more on input patch and thus performs poorer during generation.
The best results are obtained for patches retrieved by concatenating  \texttt{prev\textunderscore code} and \texttt{commit\textunderscore msg} as query.

\begin{answerbox}
\textbf{Result 2}: Retrieved patches can provide extra information
to the generation model and further improve the quality 
of the generated patch.
\end{answerbox}

Table 3 shows the baseline experiments with our hyperparameters on $B2F$ datasets without patch as an input, which is why the results slightly differ from the paper. Experiments where MODIT-generated patches as buggy line along with patch as input to CoditT5 were performed. We were able to achieve an improvement in accuracy over our CoditT5 baseline scores with input format as <buggy\_line><context> <patch> <commit>.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}


% \begin{table}[]
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{Input} & \textbf{Small Accuracy} & \textbf{Medium Accuracy} \\ \hline
% \begin{tabular}[c]{@{}l@{}}\textless{}buggy\_only\textgreater \textless{}s\textgreater \\ \textless{}prev\_code\textgreater \textless{}s\textgreater \\ \textless{}commit\_msg\textgreater{}\end{tabular} &
%   36.07\% &
%   28.74\% \\ \hline
% \begin{tabular}[c]{@{}l@{}}\textless{}buggy\_only\textgreater \textless{}s\textgreater \\ \textless{}retrieved\_patch\textgreater \textless{}s\textgreater\\ \textless{}prev\_code\textgreater \textless{}s\textgreater\\ \textless{}commit\_msg\textgreater{}\end{tabular} &
%   34.91\% &
%   28.75\% \\ \hline
% \begin{tabular}[c]{@{}l@{}}\textless{}buggy\_only\textgreater \textless{}s\textgreater\\ \textless{}prev\_code\textgreater \textless{}s\textgreater\\ \textless{}retrieved\_patch\textgreater \textless{}s\textgreater\\ \textless{}commit\_msg\textgreater{}\end{tabular} &
%   37.16\% &
%   29.99\% \\ \hline
% \end{tabular}
% \caption{Performed experiments where we passed MODIT generated patches as buggy line along with patch as input to CoditT5}
% \label{table:3}
% \end{table}


==> body/6.related_work.back.tex <==
\section{Related Work}
\textbf{Code Repair Models. } %In the past few years, 
Seq2Seq models %Neural Machine Translations (NMTs) \pelin{cite something here} 
have been studied by many researchers to repair code. Tufano \etal \cite{tufano2019empirical} introduced the encoder-decoder architecture %and NMTs 
to fix bugs. SequenceR \cite{chen2019sequencer} 
further combined %\pelin{what copy mechanism} 
copy mechanism with the $seq2seq$ model to overcome the %\pelin{what unlimited vocab problem, we never explain} 
unlimited vocabulary problem.
CocoNut \cite{lutellier2020coconut} used ensemble learning for this purpose. %on the combination of CNNs and NMT architecture 
%to improve the performance of bug fixing in multiple languages. 
%Instead of viewing source code as a sequence of tokens, 
some works treat further use tree/graph-based models~\cite{chakraborty2020codit, jiang2023knod, dinella2019hoppity}.
%or graph. Chakraborty \etal \cite{chakraborty2020codit} proposed 
% a tree-based neural network to learn bug-fixing patterns. In order to improve the accuracy of generating AST, Jiang \etal \cite{jiang2023knod} proposed a novel 3-stage decoder and incorporated it with domain knowledge.
%Hoppity \cite{dinella2019hoppity} formulated the program repair as a graph transformation problem: applying a graph edit operation on the graph representing the buggy program to produce a correct patch. Meanwhile, 


LLMs like %on code have recently shown their potential to improve models' performance on downstream tasks.
%For example, 
CodeBERT \cite{feng2020codebert}, PLBART \cite{ahmad2021unified}, CodeT5 \cite{wang2021codet5}, and NatGen \cite{chakraborty2022natgen} have 
%been evaluated on the task of program repair and have 
shown very promising results on APR. 
%MODIT \cite{chakraborty2021multi}, a multi-modal PLBART-based model, indicated that the model could benefit from extra input from developers like commit message and context information.
Fu \etal \cite{fu2022vulrepair} proposed VulRepair, a T5-based vulnerability
repair approach, to solve the limitations of previous work: VRepair \cite{chen2021neural}. 
A new trend in recent research works is using LLM in a zero-shot manner for program repair, which means that no extra training or fine-tuning is involved. %\pelin{shouldnt we say the tool name here}
Xia \etal \cite{xia2022less} directly leverages pre-trained CodeBERT \cite{feng2020codebert} to build a cloze-style APR tool.

Jiang \etal \cite{jiang2023impact} systematically evaluated 10 LLMs for APR with and without fine-tuning.
\cite{prenner2021automatic} and \cite{joshi2022repair} designed prompts for Codex \cite{chen2021evaluating} to convert code repair into code generation. 

The plastic surgery hypothesis \cite{barr2014plastic} indicates that changes to a codebase contain snippets that already exist in the codebase at the time of the change, and these snippets can be efficiently found and exploited.
However, many existed APR techniques are based on the Neural Machine Translation, which originates from the domain of Natural Language Processing, and neglect the importance of exploiting the codebase. Our proposed approach complements this line of work as we show the potential of taking any off-the-shelf APR tools and blending them with retrieval steps.


\textbf{Retrieval-based Code Repair Models.}
Some previous work focuses on finding and reusing existing code for bug repair.
ssFix \cite{xin2017leveraging} searches a code database for code snippets that
are syntactically similar to the bug context and reuses such
retrieved code snippet to synthesize patches.
sharpeFix \cite{xin2019revisiting} is built over ssFix and improves it by using different 
search methods to find candidate patches. LSRepair \cite{liu2018lsrepair} claims that code
search can speed up the process of code repair (some bugs can be fixed only in few seconds).
SimFix \cite{jiang2018shaping} builds an abstract search space and a concrete search space by mining existing patches and similar code and searches on the intersection of two spaces.
Their findings motivated us to explore if patches retrieved from the existing code base can provide more information to $seq2seq$ models and further improve their performances.

The biggest limitation of the prior pure retrieval-based methods is that their performances rely on the quality of codebase: if the pattern of code under edit / code under fix is not seen in the codebase, it can be very hard to find the patch we expect. Our proposed approach mitigates this issue by combining code search with generation model and modification model. These two components have the capability to adaptively leverage the useful information from the retrieval results and creatively synthesis patching patterns that are never seen in the existed codebase. 

\textbf{Code Editing Models}
%Different from many previous works, which model program repair with NMT, some 
Recent studies start to explore if DL models can learn explicit edit operations. 
Ding \etal\cite{ding2020patching} confirmed this claim. 
%that synthesizing edits of code conditional on the buggy context is more efficient than NMT-based models. 
Chen \etal \cite{chen2021plur} proposed to pair a 
graph encoder with a Transformer decoder to generate Tocopo sequence \cite{tarlow2020learning}, which is used to represent a code edit.
Similarly, Hephaestus \cite{connorcan2021} used an LSTM $seq2seq$ model to learn edit operations via the introduction of Levenshtein edit operations and their condensed forms: basic, strict, and loose compound operations.
%Following the huge success of the pre-trained model in the ML4Code domain, 
Zhang \etal \cite{zhang2022coditt5} designed a pre-trained model CoditT5 \cite{zhang2022coditt5} for editing tasks. 
%When fine-tuning CoditT5 \cite{zhang2022coditt5} on the task of code repair, the output is in the format of edit actions followed by fixed code. 
Different from these previous code editing models, we do not output an edit  
%our editing model in \tool does not focus on designing a certain 
 sequence directly, rather our approach slowly guides the tool towards generating the intended edit in multiple steps.
%but applies edit operations directly on the inputs in the process of transforming the buggy code to the fixed one.


Many previous works \cite{tarlow2020learning,chen2021plur,connorcan2021,zhang2022coditt5} designed special outputs to represent edit operations. For example, in the inference stage CoditT5 \cite{zhang2022coditt5} first generates an edit plan which explicitly edit operations, then it autoregressively generated the edited target sequence. In their open source implementation, since the output is composed of two parts, extra post-processing (decoding) is needed.
However, LevT does not focus on output design and directly applies explicit edit operations in the decoder. 

In practice, the generated patch is always not exactly the same as the intended patch although the code generation model has been
augmented with patch retrieval. Sometimes they are merely few tokens away. The point of the modification model in our research is to finish the ``last step" and further improve the search and generation.



==> body/CodeFig.tex <==
\begin{figure}
\begin{subfigure}{0.3\textwidth}
\begin{minted}[fontsize=\mintedfsize, escapeinside=||, linenos]{java}
// MultiplePiePlot class's constructor
public MultiplePiePlot(CategoryDataset dataset) {
  super();
|\diffdel{ setDataset(dataset);}|
|\diffadd{ this.dataset = dataset;}|
  PiePlot piePlot = new PiePlot(null);
  this.pieChart = new JFreeChart(piePlot);
  this.pieChart.removeLegend();
  ...
}
  
\end{minted}
\caption{Code Under Test.}
\vspace{10pt}
\label{Fig@OVER@MOTI@CUT}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
\begin{minted}[fontsize=\mintedfsize, escapeinside=||, linenos]{java}
public void testConstructor() {
  MultiplePiePlot plot = new MultiplePiePlot();
  assertNull(plot.getDataset());
  DefaultCategoryDataset dataset = 
    new DefaultCategoryDataset();
  plot = new MultiplePiePlot(dataset);
  // The next assert fails
  assertTrue(dataset.hasListener(plot));
  ...
}
\end{minted}
% based on https://github.com/imWildCat/scylla/blob/17e68080b799c70c9ad31846add78eaa744ca525/scylla/worker.py#L51
\caption{Failing Test-Method.}
\vspace{10pt}
\label{Fig@OVER@MOTI@FAIL}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\textwidth}
\begin{minted}[fontsize=\mintedfsize, escapeinside=||, linenos]{java}
public void testSerialization() {
  MultiplePiePlot p1 = new MultiplePiePlot(null);
  p1.setAggregatedItemsPaint(
        new GradientPaint(1.0f, ...));
  ...
  out.writeObject(p1);
  MultiplePiePlot p2 = null;
  ...
  p2 = (MultiplePiePlot) in.readObject();
  in.close();
  assertEquals(p1, p2);
}
\end{minted}
\caption{Passing Test-Method.}
\label{Fig@OVER@MOTI@PASS}
\end{subfigure}
\caption{An example of a changed code segment, and two tests covering it: one failing and one passing. The similarities between the failing test and the code-under-test are greater than that of the passing test.}
\label{Fig@OVER@MOTI} 
\end{figure}

==> body/tmp.tex <==
\section{Temporary Section for Collaboration (****TO BE REMOVED****)}

\lstset{escapechar=~,style=CustomJava}
\begin{figure*}[!htpb]
\centering
\begin{subfigure}{0.45\linewidth}
\begin{lstlisting}
int search(int[] arr, int key, int low, int high){
    while (low <= high) {
        int mid = low  + ((high - low) / 2);
        if(arr[mid] == key)  { return mid; }
        else { high = mid + 1; }
    }
    return -1;
}
\end{lstlisting}
% \vspace{-5mm}
\caption{Original Code}
\label{fig:original_code}
\end{subfigure}%
\begin{subfigure}{0.45\linewidth}
\begin{lstlisting}
int search(int[] arr, int key, int low, int high){
    ~\red{\colorbox{highlight}{\bf for}}~(~\red{\colorbox{highlight}{\bf ;}}~low <= high~\red{\colorbox{highlight}{\bf ;}}~) {
        int mid = low  + ((high - low) / 2);
        if(arr[mid] == key) { return mid; }
        else { high = mid + 1; }
    }
    return -1;
}
\end{lstlisting}
% \vspace{-5mm}
\caption{Loop Transformation}% (\S\ref{sec:loop_transformation})}
\label{fig:loop_transformation}
\end{subfigure}
\vspace{2mm}

\rule{0.95\textwidth}{0.1mm}
\begin{subfigure}{0.45\linewidth}
\begin{lstlisting}
int search(int[] arr, int key, int low, int high){
    while (low <= high) {
        int mid = low  + ((high - low) / 2);
        ~\red{\colorbox{highlight}{\bf while\quad(\quad i < \quad i \quad )\quad\{ }}~
            ~\red{\colorbox{highlight}{\bf high = mid + 1; }}~
        ~\red{\colorbox{highlight}{\bf\} }}~
        // ... Rest of the Code
    }
    return -1;
}
\end{lstlisting}
% \vspace{-5mm}
\caption{DeadCode Insertion}% (\S\ref{sec:dead_code})}
\label{fig:dead_code}
\end{subfigure}%
\begin{subfigure}{0.45\linewidth}
\begin{lstlisting}
int search(int[] arr, int key, int low, int high){
    while (~\red{\colorbox{highlight}{\bf high\quad>=\quad low}}~) {
        int mid = low  + ((high - low) / 2);
        if(~\red{\colorbox{highlight}{\bf arr$[$mid$]$\;\;$!=$\;\; key}}~)  { 
            ~\red{\colorbox{highlight}{\bf high\quad=\quad mid\;\;+\;\;1;}}~
        }
        else~\red{\colorbox{highlight}{
        \bf \{\;\;return\;\;mid;\;\;\}}}~
    }
    return -1;
}
\end{lstlisting}
% \vspace{-5mm}
\caption{Block and Operand Swap}% (\S\ref{sec:block_swap})}
\label{fig:block_swap}
\end{subfigure}
\vspace{2mm}

\rule{0.95\textwidth}{0.1mm}

\begin{subfigure}{0.45\linewidth}
\begin{lstlisting}
int search(int[] arr, int key, int low, int high){
    while (low <= high) {
        int mid = low  + ((high - low) / 2);
        if(arr[mid] == key) { return mid; }
        else { 
            high = ~\red{\colorbox{highlight}{\bf mid+\;+}}~; 
        }
    }
    return -1;
}
\end{lstlisting}
% \vspace{-5mm}
\caption{Inserting confusing code element}% (\S\ref{sec:confusion_removal})}
\label{fig:confusion}
\end{subfigure}%
\begin{subfigure}{0.45\linewidth}
\begin{lstlisting}
int search(int[] ~\red{\colorbox{highlight}{\bf var\_1}}~, int key, int low, int ~\red{\colorbox{highlight}{\bf var\_2}}~){
    while (low <= ~\red{\colorbox{highlight}{\bf var\_2}}~) {
        int mid = low  + ((~\red{\colorbox{highlight}{\bf var\_2}}~ - low) / 2);
        if(~\red{\colorbox{highlight}{\bf var\_1}}~[mid] == key) { return mid; }
        else { ~\red{\colorbox{highlight}{\bf var\_2}}~ = mid + 1; }
    }
    return -1;
}
\end{lstlisting}
% \vspace{-5mm}
\caption{Variable Renaming} % (\S\ref{sec:var_renaming})}
\label{fig:var_renaming}
\end{subfigure}
\vspace{2mm}

\rule{0.95\textwidth}{0.1mm}
% \vspace{-6mm}
\caption{Semantic preserving transformation used to prepare the pre-training data for \tool.}
%After a randomly selected noise injector injects the original code with corresponding noise, we ask the model to regenerate the original code from the noise induced code.}
\label{fig:transformations}
\end{figure*}
